Planet as a Brain: Towards Internet of AgentSites based on AIOS Server

The internet is undergoing a historical transformation from the "Internet of Websites" to the "Internet of AgentSites." While traditional Websites served as the foundation for information hosting and dissemination, a new frontier is emerging where AgentSites serve as the hubs of the internet, where each AgentSite hosts one or more AI agents that receive tasks, address them, and deliver actionable solutions, marking a significant shift in the digital landscape and representing the next generation of online ecosystems. Under this vision, AIOS, the AI Agent Operating System, serves as the server for the development, deployment and execution of AI agents, which is a fundamental infrastructure for the Internet of Agentsites. In this paper, we introduce AIOS Server, a runtime framework to host agents and enable global-scale collaboration among decentralized agents. AIOS Server provides a communication protocol leveraging the Model Context Protocol (MCP) and JSON-RPC to enable agent-agent or human-agent interactions. Each AIOS node operates as a server to host and execute agents, while supporting peer-to-peer coordination without reliance on centralized orchestration. Based on AIOS Server, we further present the world's first practically deployed Internet of Agentsites (AIOS-IoA), including AgentHub for agent registration and discovery and AgentChat for interactive communication, at https://planet.aios.foundation. The agent discovery mechanism based on Distributed Hash Tables (DHT) and a Gossip protocol serves as the search engine for the internet of agentsites. This work provides a practical foundation for building the Internet of Agentsites-a new paradigm where autonomous agents become first-class citizens of the web. The implementation is available at https://github.com/agiresearch/AIOS.Server and is integrated into the AIOS main branch at https://github.com/agiresearch/AIOS.

==> sections/acknowledge.tex <==
\section{Acknowledgment}

We would like to thank the anonymous reviewers for their constructive feedback and the members of our test group for their valuable insights. Special thanks go to the LaTeX community for developing the tools and packages that made this project possible. Additionally, we extend our gratitude to Qwen and DeepSeek for their invaluable contributions to the development of this template. Their expertise in natural language processing and code generation greatly accelerated the project timeline and ensured the highest level of quality.


==> sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

This paper presents a clean, unified, and aesthetically pleasing LaTeX template for arXiv submissions. By combining rigorous design principles with practical implementation details, our template simplifies the manuscript preparation process while improving the visual quality of published works. With significant contributions from AI models Qwen and DeepSeek, we were able to incorporate innovative features that enhance both functionality and user experience. Initial evaluations suggest that it meets the needs of a wide range of researchers, making it a valuable resource for the academic community.

We hope that this contribution will inspire further efforts toward standardizing and enhancing the presentation of scientific knowledge on platforms like arXiv.


==> sections/discussions.tex <==
\vspace{-2mm}
\section{Discussions}

While our template addresses many challenges associated with arXiv submissions, several limitations remain. First, some advanced LaTeX users may prefer more granular control over formatting than our template currently offers. Second, although we aimed for broad compatibility, certain edge cases—such as highly specialized equation rendering—may require additional adjustments.

Future work could focus on expanding the template's feature set, integrating support for alternative markup languages (e.g., Markdown), and exploring machine learning techniques to automate parts of the formatting process. Continued collaboration with AI models like Qwen and DeepSeek will be crucial in realizing these advancements.

==> sections/experiments.tex <==
\vspace{-2mm}
\section{Experiments}

To evaluate the effectiveness of our template, we conducted two sets of experiments:

\begin{itemize}[leftmargin=7mm,itemsep=2mm, topsep=0em]
    \item[1.] Qualitative Assessment : A panel of ten researchers from various disciplines reviewed sample papers formatted with our template. They rated each document on readability, visual appeal, and overall satisfaction.
    \item[2.] User Feedback : We distributed the template to a group of 20 graduate students and early-career researchers, asking them to prepare mock submissions and provide feedback on usability and customization.
\end{itemize}

Results indicate that participants found the template intuitive and effective, with average satisfaction scores exceeding 85\%. Common praises included "professional appearance" and "ease of modification." Several users specifically noted how seamlessly the AI-generated components integrated into the template.


==> sections/introduction.tex <==
\vspace{-4mm}
\section{Introduction}

The dissemination of research findings is a critical component of academic progress, and arXiv plays an indispensable role in facilitating this process. Despite its widespread adoption, many authors struggle with formatting their manuscripts due to the absence of an official, universally accepted template. As a result, arXiv submissions vary significantly in style, structure, and visual appeal, which can detract from the clarity and professionalism of the work presented.

\begin{center}
\emph{
Towards a Clean, Unified, and Aesthetically Pleasing arXiv Template
}
\end{center}

To address this issue, we propose a novel LaTeX-based template that prioritizes three key objectives: (1) cleanliness, ensuring minimal distractions caused by unnecessary design elements; (2) unification, promoting consistency across different papers; and (3) aesthetic appeal, enhancing the visual experience for readers. The development of this template was made possible through close collaboration with two state-of-the-art AI assistants, Qwen~\cite{hui2024qwen2} and DeepSeek~\cite{guo2025deepseek}, whose capabilities in natural language processing and code generation were instrumental in achieving our goals. By adhering to these principles, our template aims to streamline the submission process and improve the overall quality of published works on arXiv.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/figure1.png}
    \vspace{-10mm}
    \caption{We collaborated with Qwen and DeepSeek to complete this arxiv template.}
    \label{fig:overall_figure}
\end{figure}

\label{sec:intro}
\vspace{-1mm}


==> sections/method.tex <==
\section{Method}
\label{sec:method}

\subsection{Design Principles}

Our template is guided by three core design principles:

\begin{itemize}[leftmargin=7mm,itemsep=2mm, topsep=0em]
    \item Cleanliness : The layout avoids clutter and focuses on content readability.
    
    \item Unification : Consistent typography, spacing, and sectioning ensure that all papers using the template share a common identity.
    
    \item Aesthetic Appeal : Thoughtful use of whitespace, font choices, and color schemes enhances the visual impact without overwhelming the reader.
\end{itemize}

\subsection{Design Principles}

The template is implemented in LaTeX, leveraging modern packages such as geometry, fontspec, and microtype to achieve precise control over page layout and typography. Key features include:

\begin{itemize}[leftmargin=7mm,itemsep=2mm, topsep=0em]
    \item Automatic generation of title pages and metadata.
    
    \item Support for multi-column layouts, figures, tables, and mathematical equations.
    
    \item Customizable options for author affiliations, abstract placement, and bibliographies.
\end{itemize}

Additionally, we provide detailed documentation and sample files to help users quickly adapt the template to their specific needs.

\textbf{Collaboration with Qwen and DeepSeek}

In developing this template, we collaborated extensively with two powerful AI models: Qwen~\footnote{\url{https://qwen.ai}} and DeepSeek~\footnote{\url{https://chat.deepseek.com}}. Their contributions included:

\begin{itemize}[leftmargin=7mm,itemsep=2mm, topsep=0em]
    \item[1.] Automated Code Generation : Both Qwen and DeepSeek assisted in generating efficient and error-free LaTeX code snippets, reducing manual coding time and ensuring high-quality implementation.
    
    \item[2.] Semantic Content Structuring : Using their advanced natural language understanding capabilities, Qwen and DeepSeek helped optimize the logical flow of sections and subsections, ensuring that the template adheres to best practices for academic writing.
    
    \item[3.] Layout Optimization : Through iterative refinement, Qwen and DeepSeek analyzed feedback from early testers to suggest improvements in whitespace usage, figure placement, and table formatting, resulting in a more polished final product.
\end{itemize}

These AI-driven enhancements allowed us to create a template that not only meets technical requirements but also offers a superior user experience.



==> sections/relatedwork.tex <==
\section{Related Work}
\label{sec:related_work}

Previous efforts to standardize document preparation for academic publishing have primarily focused on journal-specific templates or proprietary software solutions. For example, Elsevier and Springer provide LaTeX templates tailored to their respective journals, but these are not suitable for open-access platforms like arXiv. Similarly, tools such as Overleaf offer collaborative environments for writing LaTeX documents, yet they do not enforce uniformity or aesthetics.

Some community-driven initiatives have attempted to create general-purpose templates for arXiv. Notable examples include the arxiv-style package and custom templates shared via GitHub repositories. While these resources are valuable, they often lack comprehensive documentation, flexibility, or attention to visual design. Our work builds upon these foundations by incorporating best practices from both academia and graphic design, further enhanced by leveraging cutting-edge AI technologies provided by Qwen and DeepSeek.

